JWST MIRI detections of H$\alpha$ and [O III] and direct metallicity measurement of the $z=10.17$ lensed galaxy MACS0647$-$JD

JWST spectroscopy has revolutionized our understanding of galaxies in the early universe. Covering wavelengths up to $5.3\,{\rm \mu m}$, NIRSpec can detect rest-frame optical emission lines H$\alpha$ out to $z = 7$ and [O III] to $z = 9.5$. Observing these lines in more distant galaxies requires longer wavelength spectroscopy with MIRI. Here we present MIRI MRS IFU observations of the lensed galaxy merger MACS0647$-$JD at $z = 10.165$. With exposure times of 4.2 hours in each of two bands, we detect H$\alpha$ at $9\sigma$, [O III]$\,\lambda5008$ at $11\sigma$, and [O III]$\,\lambda4960$ at $3\sigma$. Combined with previously reported NIRSpec spectroscopy that yields seven emission lines including the auroral line [O III]$\,\lambda4363$, we present the first direct metallicity measurement of a $z > 10$ galaxy: $12+{\rm log(O/H)}= 7.79\pm0.09$, or $0.13^{+0.02}_{-0.03}\,Z_{\odot}$. This is similar to galaxies at $z \sim 4 - 9$ with direct metallicity measurements, though higher than expected given the high specific star formation rate ${\rm log(sSFR / yr^{-1})} = -7.4 \pm 0.3$. We further constrain the ionization parameter ${\rm log}(U)$ = $-1.9 \pm 0.1$, ionizing photon production efficiency ${\rm log}(\xi_{\rm ion})$ = $25.3\pm0.1$, and star formation rate $5.0\pm0.6\,M_{\odot}/{\rm yr}$ within the past $10\,{\rm Myr}$. These observations demonstrate the combined power of JWST NIRSpec and MIRI for studying galaxies in the first $500$ million years.

==> flux.tex <==
% Filters
\begin{deluxetable*}{lccrrrc}
\tablecaption{\label{tab:photometry}Measured MIRI photometry for MACS0647$-$JD, JDA, and JDB.
}
\tablewidth{\columnwidth}
\tablehead{
\colhead{Emission Lines/Filters} &
\colhead{Rest wavelength} &
\colhead{Observed wavelength} &
\colhead{MACS0647$-$JD} &
\colhead{JDA$^{a}$} &
\colhead{JDB$^{a}$} &
\vspace{-0.07in}\\
\colhead{} &
\colhead{$\rm \AA$}  &
\colhead{$\rm \mu m$} &
\multicolumn{3}{c}{${\rm \mu Jy}$} 
%\colhead{$10^{-19}\,$erg/s/cm$^2$} &
%\colhead{$10^{-19}\,$erg/s/cm$^2$} &
%\colhead{$10^{-19}\,$erg/s/cm$^2$} 
}
\startdata
%\CIIIdw
F560W Flux$^{c}$
& $\sim5015$
& 5.6
& $0.48\pm0.04$
& $0.19\pm0.03$
& $0.22\pm0.03$\\
F770W Flux$^{c}$
& $\sim6895$
& 7.7
& $0.32\pm0.03$
& 
& \\
\enddata
\tablenotetext{a}{We refer the blue (brighter) component seen in H$\alpha$ (Figure \ref{fig:velocity}) as JDB while the red (fainter) component as JDA.}
\tablenotetext{b}{MIRI MRS spectroscopy is of JD1, JD1A, and JD1B, which is not corrected for lensing ($\mu=8$).}
\tablenotetext{c}{MIRI photometry is of JD2, JD2A, and JD2B, which is not corrected for lensing ($\mu=5.3$).}
%\tablecomments{
%\cite{Hopkins10} find maximum stellar mass density $10^{11} M_\odot$ kpc$^{-2}$ = $10^5 M_\odot$ pc$^{-2}$.
%We're just below that.
%SMGs $> 1000 M_\odot$ yr$^{-1}$ kpc$^{-2}$. We're also below that.
%}
\end{deluxetable*}
% https://docs.google.com/spreadsheets/d/1k5Xgf7vtZjnpvPa5rycbFL_WlGYhXsqBX5VMnrCTFos


==> lineflux.tex <==
% Filters
\begin{deluxetable*}{lccrrrc}
\tablecaption{\label{tab:lines}Measured emission line fluxes in MIRI MRS and MIRI photometry for MACS0647$-$JD, JDA, and JDB.
}
\tablewidth{\columnwidth}
\tablehead{
\colhead{Emission Lines/Filters} &
\colhead{Rest wavelength} &
\colhead{Observed wavelength} &
\colhead{MACS0647$-$JD} &
\colhead{JDA$^{a}$} &
\colhead{JDB$^{a}$} &
\vspace{-0.07in}\\
\colhead{} &
\colhead{$\rm \AA$}  &
\colhead{$\rm \mu m$} &
\multicolumn{3}{c}{$10^{-19}\,$erg/s/cm$^2$ and ${\rm \mu Jy}$} 
%\colhead{$10^{-19}\,$erg/s/cm$^2$} &
%\colhead{$10^{-19}\,$erg/s/cm$^2$} &
%\colhead{$10^{-19}\,$erg/s/cm$^2$} 
}
\startdata
%\CIIIdw
\OIII$^{b}$%\,\lambda4363
& 5008 
& 5.59
& $78\pm9$
& $<22\pm7$
& $78\pm9$ \\
H$\alpha$$^{b}$
& 6563
& 7.33
& $58\pm6$
& $22\pm6$
& $36\pm4$\\
F560W Flux$^{c}$
& $\sim5015$
& 5.6
& $0.42\pm0.04$
& $0.19\pm0.03$
& $0.22\pm0.03$\\
F770W Flux$^{c}$
& $\sim6895$
& 7.7
& 
& \\
\enddata
\tablenotetext{a}{We refer the blue (brighter) component seen in H$\alpha$ (Figure \ref{fig:velocity}) as JDB while the red (fainter) component as JDA.}
\tablenotetext{b}{MIRI MRS spectroscopy is of JD1, JD1A, and JD1B, which is not corrected for lensing ($\mu=8$).}
\tablenotetext{c}{MIRI photometry is of JD2, JD2A, and JD2B, which is not corrected for lensing ($\mu=5.3$).}
%\tablecomments{
%\cite{Hopkins10} find maximum stellar mass density $10^{11} M_\odot$ kpc$^{-2}$ = $10^5 M_\odot$ pc$^{-2}$.
%We're just below that.
%SMGs $> 1000 M_\odot$ yr$^{-1}$ kpc$^{-2}$. We're also below that.
%}
\end{deluxetable*}
% https://docs.google.com/spreadsheets/d/1k5Xgf7vtZjnpvPa5rycbFL_WlGYhXsqBX5VMnrCTFos


==> lines1.tex <==
% Filters
\begin{deluxetable*}{lcccccc}
\tablecaption{\label{tab:lines}MIRI MRS measured emission line fluxes for \JD1.
}
\tablewidth{\columnwidth}
\tablehead{
\colhead{Emission} &
\colhead{Rest} &
\colhead{Observed} &
\colhead{Redshift} &
\colhead{Observed} &
\colhead{Observed} &
\colhead{Intrinsic} 
\\[-0.2cm]
%\vspace{-0.07in}
%\\
\colhead{Line} &
\colhead{wavelength} &
\colhead{wavelength} &
\colhead{$z$} &
\colhead{Flux\supa} &
\colhead{FWHM} &
\colhead{FWHM}
\\[-0.2cm]
\colhead{} &
\colhead{$\rm \AA$}  &
\colhead{$\rm \mu m$} &
\colhead{} &
\colhead{$10^{-19}\,$erg/s/cm$^2$} &
\colhead{\kms} &
\colhead{\kms}
%
%\multicolumn{3}{c}{$10^{-19}\,$erg/s/cm$^2$} 
%\colhead{$10^{-19}\,$erg/s/cm$^2$} &
%\colhead{$10^{-19}\,$erg/s/cm$^2$} 
}
\startdata
%\CIIIdw
\OIII %$^{b}$%\,\lambda4363
& 5008.22 
& $5.5922 \pm 0.0002$
& $10.1660 \pm 0.0004$
& $78\pm9$
& $126\pm14$
& $99\pm11$
\\
\Halpha\ (two Gaussians)  % $^{b}$
& 6564.62
& 
& 
& $58\pm6$
& 
& 
\\
\Halpha\ blue peak
& 6564.62
& $7.3297 \pm 0.0002$
& $10.1655 \pm 0.0003$
& $36\pm4$
& $128\pm15$\supb
& $99\pm12$
\\
\Halpha\ red peak
& 6564.62
& $7.3334 \pm 0.0004$
& $10.1711 \pm 0.0007$
& $22\pm6$
& $139\pm35$
& $113\pm35$
\\
\Halpha\ (single Gaussian)
& 6564.62
& $7.3308 \pm 0.0003$
& $10.1671 \pm 0.0005$
& $55\pm6$
& $213\pm28$
& $197\pm26$
\enddata
%\tablenotetext{a}{We refer the blue (brighter) component seen in H$\alpha$ (Figure \ref{fig:velocity}) as JDB while the red (fainter) component as JDA.}
\tablenotetext{a}{JD1 line fluxes are not corrected for lensing magnification ($\mu=8$).}
\tablenotetext{b}{FWHM fixed to that of \OIII\ within 2 \kms.}
%\tablenotetext{c}{MIRI photometry is of JD2, JD2A, and JD2B, which is not corrected for lensing ($\mu=5.3$).}
%\tablecomments{
%\cite{Hopkins10} find maximum stellar mass density $10^{11} M_\odot$ kpc$^{-2}$ = $10^5 M_\odot$ pc$^{-2}$.
%We're just below that.
%SMGs $> 1000 M_\odot$ yr$^{-1}$ kpc$^{-2}$. We're also below that.
%}
\end{deluxetable*}
% https://docs.google.com/spreadsheets/d/1k5Xgf7vtZjnpvPa5rycbFL_WlGYhXsqBX5VMnrCTFos


==> properties.tex <==
% Filters
\begin{deluxetable*}{ccccc}
\tablecaption{\label{tab:phys}Line Ratios and Physical properties estimated for MACS0647$-$JD.}
\tablewidth{\columnwidth}
\tablehead{
\colhead{MACS0647$-$JD} &
\colhead{} &
\colhead{} &
%\colhead{Total}&
%\colhead{Total}
\multicolumn{2}{c}{Normalized to H$\alpha$/H$\gamma$=6.11} \\[-0.2cm]
%\colhead{JDA} &
%\colhead{JDB} \\
\colhead{Emission lines used} &
\colhead{Stacked$^{a}$} &
\colhead{Obs 21 JD2} &
\colhead{Stacked} &
\colhead{Obs 21 JD2}}
%\colhead{Obs 21 JD1} &
%\colhead{Obs 21 (JD2$-$JD1)}}
\startdata
%\CIIIdw
\multicolumn{5}{c}{Line Ratios} \\ \hline
\OIIIw\ $/$ $\lambda$4363 & $25\pm9$ & $24\pm15$  & $25\pm9$ & $32\pm18$  \\% &31&43\\
O32 = \OIIIw\ $/$ \OIIw\ & $15\pm3$& $9\pm1$ & $15\pm1$ & $11\pm1$ \\%&8 &16\\
%O32 & $7.31\pm0.14$ \\
H$\alpha$ / H$\gamma$ & $6.2\pm1.1$  & $4.7\pm0.7$ &  \multicolumn{2}{c}{6.11 (fixed)}\\% & 6.11 \\%$10.0$ & $6.0$ \\
R3 = \OIIIw\ $/$ H$\beta$ & \multicolumn{4}{c}{$3.7\pm0.6$}\ \\%$<3.5$ &$6.0\pm1.0$\\
\hline \hline   
%Stellar mass & log($M_*$) & $10^{7}\,M_{\odot}$ \\
%Escape fraction & $f_{\rm esc}$ \\
\multicolumn{5}{c}{Physical Properties} \\ \hline  12+log(O/H)$^{b}$ & $7.34\pm0.14$ & $7.40\pm0.17$ & $7.34\pm0.14$ & $7.46\pm0.19$ \\ %$7.19?$ & $7.5\pm0.2$\\
%\pyneb\ 12+log(O/H) & $7.31\pm0.14$ \\
log($U$) & $-1.9\pm0.1$ &$-2.1\pm0.1$&$-1.9\pm0.1$& $-2.0\pm0.1$\\% $-1.8?$ & $-1.8\pm0.1$ \\
SFR ($M_{\odot}\,{\rm yr^{-1}}$) &  \multicolumn{4}{c}{$3.2\pm0.3$}\\% & $3.5\pm0.4$ \\%& $1.2\pm0.3$ & $2.0\pm0.2$\\
%EW(H$\alpha$) \\
log(\xiion) & \multicolumn{4}{c}{$25.1\pm0.1$}\\
$T_{e}(\rm{[OIII]})$(K) & $21000\pm2700$ & $21000\pm3000$ & $21000\pm2700$ & $19000\pm3100$ 
\enddata
\tablenotetext{a}{We adopt this configuration as fiducial values throughout the letter.}
\tablenotetext{b}{Estimated using \pyneb.}
%\tablecomments{
%\cite{Hopkins10} find maximum stellar mass density $10^{11} M_\odot$ kpc$^{-2}$ = $10^5 M_\odot$ pc$^{-2}$.
%We're just below that.
%SMGs $> 1000 M_\odot$ yr$^{-1}$ kpc$^{-2}$. We're also below that.
%}
\end{deluxetable*}
% https://docs.google.com/spreadsheets/d/1k5Xgf7vtZjnpvPa5rycbFL_WlGYhXsqBX5VMnrCTFos

